Evolving 5G: ANIARA, an Edge-Cloud perspective

Emerging use-cases like smart manufacturing and smart cities pose challenges in terms of latency, which cannot be satisfied by traditional centralized networks. Edge networks, which bring computational capacity closer to the users/clients, are a promising solution for supporting these critical low latency services. Different from traditional centralized networks, the edge is distributed by nature and is usually equipped with limited connectivity and compute capacity. This creates a complex network to handle, subject to failures of different natures, that requires novel solutions to work in practice. To reduce complexity, more lightweight solutions are needed for containerization as well as smart monitoring strategies with reduced overhead. Orchestration strategies should provide reliable resource slicing with limited resources, and intelligent scaling while preserving data privacy in a distributed fashion. Power management is also critical, as providing and managing a large amount of power at the edge is unprecedented.

==> WP1.tex <==
%
% WP1
%
% \section{ANIARA’s use cases} 
% \label{section_WP1}



% \subsection{Smart Manufacturing Use Cases}
% At the industrial level, manufacturing requirements have become more challenging. Digitalization of data, with low latency, high frequency and connectivity, while generating new insights through AI has been driving the future of industrial decision making. 

% Industrial application requirements hover on the shop floor plane for more innovative automation, networking and connectivity solutions for smart edge devices. These devices, responsible for data acquisition, pre-processing, broadcasting and more, are a key point of the industrial use cases for their critical influence in manufacturing processes.

% At an edge cloud level, automation and (micro-)services management are becoming more complex. Also, security aspects are taking increasingly part on the requirements. With respect to this, the application requirements are demanding scalable edge-cloud environments, higher AI-on-the-edge resource availability and secure network between production plants and IT-infrastructure.

% \subsection{Smart City Use Cases}

